Improved Algorithm for Min-Cuts in Distributed Networks

In this thesis, we present fast deterministic algorithm to find small cuts in distributed networks. Finding small min-cuts for a network is essential for ensuring the quality of service and reliability. Throughout this thesis, we use the CONGEST model which is a typical message passing model used to design and analyze algorithms in distributed networks. We survey various algorithmic techniques in the CONGEST model and give an overview of the recent results to find cuts. We also describe elegant graph theoretic ideas like cut spaces and cycle spaces that provide useful intuition upon which our work is built. Our contribution is a novel fast algorith to find small cuts. Our algorithm relies on a new characterization of trees and cuts introduced in this thesis. Our algorithm is built upon several new algorithmic ideas that, when coupled with our characterization of trees and cuts, help us to find the required min-cuts. Our novel techniques include a tree restricted semigroup function (TRSF), a novel sketching technique, and a layered algorithm. TRSF is defined with respect to a spanning tree and is based on a commutative semigroup. This simple yet powerful technique helps us to deterministically find min-cuts of size one (bridges) and min-cuts of size two optimally. Our sketching technique samples a small but relevant vertex set which is enough to find small min-cuts in certain cases. Our layered algorithm finds min-cuts in smaller sub-graphs pivoted by nodes at different levels in a spanning tree and uses them to make the decision about the min-cuts in the complete graph. This is interesting because it enables us to show that even for a global property like finding min-cuts, local information can be exploited in a coordinated manner.

==> synopsis_subparts/characterization.tex <==
%TEX root = ../soda_17.tex
In this section, we will establish some fundamental relationships between trees and cuts which will help us find the required min-cuts. When a min-cut shares $k$ edges with a spanning tree then we say that it $k$-respects the tree. Each min-cut will at least share one edge with a spanning tree.


For any node $v$ and a tree $T$, let $\desc[T]{v}$ be the vertex set which includes $v$ and its decedents in the tree $T$. For any node $v\neq r$ let $\ancestor[T]{v}$ be the ancestor of node $v$, $\level[T]{v}$ be the depth of node $v$ with root $r$ being at level $0$ and $\child_T(v)$ be the children of node $v$ in the tree $T$. For each node $v \neq r$, let $\parent[T]{v}$ be the parent of node $v$ in the tree $T$. For any vertex set $A \subset V$, let $\delta(A)$ be the set of edges which are in the cut $(A,V\setminus A)$. We use the following result about cut spaces \citep{bondy1976graph} to prove our characterizations.

\begin{lemma}
\label{main-lemma}
Let $A_1,A_2,\ldots, A_j$ be set of vertices such that $\forall i\ A_i \subset V$ then $\delta(A_1 \oplus A_2 \oplus \ldots \oplus A_j) = \delta(A_1) \oplus \delta(A_2) \oplus \ldots \oplus \delta(A_j)$
\end{lemma}

For any $A,B \subseteq V$, let $\gamma(A,B) = |\delta(A) \cap \delta(B)|$. We give the following lemma to characterize the induced cuts of size 2 such that it 2-respects a tree $T$.

% % % % % % % % % % % % % % % % % % % % % % % % % % % %
% % % % Begin: Characterizing Lemma about 2-cuts % % % %
% % % % % % % % % % % % % % % % % % % % % % % % % % % %

\begin{lemma}
\label{lemma:2-respect-2-cut}
Let $T$ be any tree. When $u \neq v$ and $u,v \in V\setminus r$. Then the following two statements are equivalent.
\begin{enumerate}[$P_1:$]
\item $\curly{(\parent[T] u,u),(\parent[T] v,v)}$ is a cut set induced by ${\desc[T]{u}}\oplus {\desc[T]{v}}$.
\item $|\delta(\desc[T]{u})| = |\delta(\desc[T]{v})| = \gamma({\desc[T]{u}},{\desc[T]{v}}) + 1$
\end{enumerate}
\end{lemma}
To prove the above lemma the following simple observation will be helpful
\begin{obs}
\label{obs:simple_observation_2_cuts}
For any $u\neq v$ and $u,v \in V\setminus r$, the edge $(\parent[T]{v},v) \in \delta({\desc[T]{v}})$  but $(\parent[T]{v},v) \notin \delta({\desc[T]{u}})$; also $(\parent[T]{u},u) \in \delta({\desc[T]{u}})$  but $(\parent[T]{u},u) \notin \delta({\desc[T]{v}})$.
\end{obs}
\begin{proof}[Proof of Lemma \ref{lemma:2-respect-2-cut}]
Consider the forward direction, $\curly{(\parent[T] u,u),(\parent[T]v,v)}$ is a cut set induced by ${\desc[T]{u}}\oplus {\desc[T]{v}}$. Therefore $\delta({\desc[T]{v}} \oplus {\desc[T]{u}}) = \curly{(\parent[T]u,u),(\parent[T]v,v)}$. Further from Lemma \ref{main-lemma}, we have $\delta({\desc[T]{v}} \oplus {\desc[T]{u}})=\delta({\desc[T]{u}}) \oplus \delta({\desc[T]{v}})$. Therefore $\curly{(\parent[T]u,u),(\parent[T]v,v)} = \delta({\desc[T]{u}}) \oplus \delta({\desc[T]{v}})$ which along with Observation \ref{obs:simple_observation_2_cuts} implies that $\delta({\desc[T]{u}})\setminus (\parent[T]{u},u) = \delta({\desc[T]{v}})\setminus(\parent[T]{v},v)$ thus $|\delta({\desc[T]{v}})|-1 = |\delta({\desc[T]{v}}) \cap\delta({\desc[T]{u}})|$ and $|\delta({\desc[T]{u}})|- 1= |\delta({\desc[T]{v}}) \cap\delta({\desc[T]{u}})|$. 

For the other direction, given that $|\delta({\desc[T]{u}}) \cap \delta({\desc[T]{v}})| + 1 = |\delta({\desc[T]{v}})| = |\delta({\desc[T]{u}})|$, which along with Observation \ref{obs:simple_observation_2_cuts} implies that $\delta({\desc[T]{u}})\setminus (\parent[T]{u},u) = \delta({\desc[T]{v}})\setminus (\parent[T]{v},v)$. Hence $\delta({\desc[T]{u}}) \oplus \delta({\desc[T]{v}}) = \curly{(\parent[T]{u},u),(\parent[T]{v},v)}$. Using the fact that $\delta({\desc[T]{v}}) \oplus \delta({\desc[T]{u}}) = \delta({\desc[T]{v}} \oplus {\desc[T]{u}})$; the edge set $\curly{(\parent[T]u,u),(\parent[T]v,v)}$ is a cut induced by ${\desc[T]{v}} \oplus {\desc[T]{u}}$. 
\end{proof}
% % % % % % % % % % % % % % % % % % % % % % % % % % % %
% % % % End: Characterizing Lemma about 2-cuts % % % %
% % % % % % % % % % % % % % % % % % % % % % % % % % % %
Similar to the above lemma, we also characterize min-cuts of size 3 which 2-respects the tree and a min-cut of size $3$ which 3 respects the tree. Detailed proofs of these lemmas are given in the thesis.
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% % % % % % % Begin: 3-cut which 2 respect% % % % % % % % % % % % 
% % % % % % % Characterizing Lemma Introduction % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\begin{lemma}
Let $T$ be any tree. Let $v_1,v_2 \in V\setminus r$ be two different nodes and $e$ be a non-tree edge, then the following two are equivalent
\begin{enumerate}[$P_1:$]
\item $\curly{(\parent[T]{v_1},v_2),(\parent[T]{v_2},v_2),e}$ is a cut set induced by the vertex set $\desc[T]{v_1}\oplus \desc[T]{v_2}$
\item $|\delta(\desc[T]{v_1})| -2 = |\delta(\desc[T]{v_2})| -1 = \gamma({\desc[T]{v_1}},{\desc[T]{v_2}})$ or $\delta(\desc[T]{v_1}) -1 = |\delta(\desc[T]{v_2})| -2 = \gamma({\desc[T]{v_1}},{\desc[T]{v_2}})$ 
\end{enumerate}
\label{lemma:gen_3_cut_2_respect}
\end{lemma}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% % % % % % % Begin: Characterizing Lemma % % % % % % % % % % % % 
% % % % % % % Lemmas. for 3-cut 3-respect % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\begin{lemma}
\label{lemma:gen_3_cut_3_respect}
Let $T$ be any tree. Let $v_1,v_2,v_3 \in V\setminus r$, further each of $v_1,v_2$ and $v_3$ are different then the following two statements are equivalent
\begin{enumerate}[$P_1:$]
\item $\curly{(v_1,\parent[T]{v_1}),(v_2,\parent[T]{v_2}),(v_3,\parent[T]{v_3})}$ is a cut-set induced by $\desc[T]{v_1}\oplus \desc[T]{v_2} \oplus \desc[T]{v_3}$
\item $|\delta(\desc[T]{v_i})| -1 = \sum\limits_{j \in \curly{1,2,3}\setminus i}\gamma(\desc[T]{v_i},\desc[T]{v_j}),\ \forall i \in \curly{1,2,3}$
\end{enumerate}
\end{lemma}

We will work with an arbitrary BFS tree $\tree$ of the given network. Whenever a quantity is computed with respect to this BFS tree $\tree$, we will skip the redundant $\tree$ from the subscript or superscript, for example $\parent{v}$ instead of $\parent[\tree]{v}$ and $\desc{v}$ instead of $\desc[\tree]{v}$. At the beginning each node $v\neq r$ knows $\level{v}$, $\parent{v}$ and the ancestor set $\ancestor{v}$. These quantities and the BFS tree can be fixed in the beginning in $O(D)$ rounds \citep{peleg2000distributed}.

==> synopsis_subparts/futureWork.tex <==
%TEX root = ../synopsis.tex
We have discussed an overview of techniques for finding min-cut. Before our result, a decade old work existed to find small min-cuts by \cite{pritchard2008fast}. They gave an algebraic technique of random circulation for finding min-cut of size $1$ and $2$. On the contrary, we give deterministic and purely combinatorial techniques for finding min-cuts of size $1,2$ and $3$. Our algorithm takes $O(D)$ rounds for finding min-cut of size $1,2$ and $O(D^2)$ rounds for finding min-cut of size $3$. An immediate future goal could be to prove that the lower bound $O(D^2)$ for a min-cut of size $3$ which is not trivial.

Currently, there are some fundamental issues for finding min-cuts of size $4$ and above using our techniques. It would be very interesting to extend our techniques for min-cut of size $4$. We are hopeful about it and give the following conjecture

\begin{conj}
There exists a distributed algorithm which can find a min-cut of size $k$ in $O(D^k)$ rounds.
\end{conj}

==> synopsis_subparts/introduction.tex <==
%TEX root = ../synopsis.tex
Networks of massive sizes are all around us. From large computer networks which are
the backbone of the internet to sensor networks of any manufacturing unit, the ubiquity of these networks cannot be denied. Each node in these kinds of networks is an independent compute node or abstracted as one. Further, nodes in these networks only have knowledge of their immediate neighbors, but not the whole topology. There are many applications which require us to solve problems related to such networks. To solve such problems, a trivial idea is as follows: Each node sends its adjacency list to one particular node through the underlying communication network; that node then finds the required property using the corresponding sequential algorithm. Such an idea may not be cost effective due to the constraints of the capacity of links and large sizes of these networks.  The question then is: Does there exist a faster cost-effective algorithm through which nodes in a network can coordinate among each other to find the required network property? Such a question is part of a more generalized spectrum of \emph{Distributed Algorithms}. 

We give a fast distributed algorithm for finding small min-cuts. An edge cut is the set of edges whose removal disconnects the network. An edge cut with a minimum number of edges is called as a \emph{min-cut}. Our approach to find the min-cut is based on our novel distributed algorithmic techniques and backed by new characterizations of cuts and trees. Our algorithmic techniques are as follows:
\begin{itemize}
\item \emph{Tree Restricted Semigroup Function} wherein a semigroup function is computed for each node in the network based on a rooted spanning tree
\item \emph{Sketching Technique} which allows us to sample small but relevant information of the network in a fast and efficient manner 
\item \emph{Layered Algorithm} which finds min-cuts in smaller sub-graphs and strategically uses the information to make the decision about min-cuts in the complete graph.
\end{itemize}


\subsection{Notations and Conventions}
We consider an undirected, unweighted and simple graph $G = (V,E)$ where $V$ is the vertex set and $E$ is the edge set. Edges are the underlying physical links and vertices are the compute nodes in the network. We will use the term vertex and node interchangeably. Similarly, edges and links will be used interchangeably. 

A cut $C = (A,V\setminus A)$, where $\emptyset \subsetneq A \subsetneq V$ is a partition of the vertices into two parts. The cut-set is the edges crossing these two parts. A min-cut is a cut-set with a minimum number of edges. Let $d_G(u,v)$ be the distance between any two nodes $u,v$ which is defined by the number of edges in the shortest path between them. We will consider connected networks, so $d_G(u,v)$ is guaranteed to be well defined and finite. The diameter of the graph $G$ is defined as $\max\limits_{u,v \in V} d_G(u,v)$. We will use $D$ to denote the diameter of the graph and $n$ for the number of vertices. 

In a typical communication network, the diameter $D$ is much smaller than the number of vertices $n$. This is because the networks are designed in a way such that any message sent from a node to any other node should not pass through too many links.

\subsection{Distributed Model}
Different types of communication networks have different parameters. This is primarily based on how communication takes place between any two nodes in a distributed system.  For the algorithm designers, these details are hidden and abstracted by appropriate modeling of the real world scenario. An established book in this domain titled \lq Distributed Computing: A Locality Sensitive Approach\rq\ \citep{peleg2000distributed} remarks: \lq\lq\emph{The number of different models considered in the literature is only slightly lower than the number of papers published in this field}". But certainly, over the years, the research community working around this area have narrowed down to a handful of models. Out of them, the \CONGEST model has been quite prominent and captures several key aspects of typical communication networks.

In the \CONGEST model, as in most other distributed networks, each vertex acts as an independent compute node. Two nodes may communicate to each other in synchronous rounds only if they have a physical link between them. The message size is restricted to $O(\log n)$ bits across each link in any given round. We will focus our attention on communication which is more expensive than computation. 

In the \CONGEST model, the complexity of an algorithm is typically measured in terms of the number of rounds required for an algorithm to terminate. Parallels of this could be drawn to the time complexity of sequential algorithms. Much of the focus has been on the study of the distributed round complexity of algorithms but recently there have been some renewed interest to study the message complexity (the sum total of messages transmitted across all edges) as well \citep{Pandurangan:2017:TMD:3055399.3055449,Elkin:2017:SDD:3087801.3087823}. Apart from these some recent research is also being directed towards the study of asymptotic memory required at each node during the execution of the algorithm \citep{DBLP:journals/corr/ElkinN17}.
We will focus on the analysis of round complexity. 

\subsection{Classification based on locality}
Any problem pertaining to a communication network may depend either on local information or global information. Local information of a node comprises knowledge of immediate neighbors or nodes which are just a constant number of hops away. Global information includes knowledge of nodes across the network.

One of the prominent examples of a problem which just requires local information is of finding a \emph{maximal independent set} (MIS). An \emph{indpendent set} is a set of vertices such that no two vertices in the set have an edge between them. An MIS is an independent set such that no vertex can be added into it without violating independence. It has been shown by \cite{Luby:1985:SPA:22145.22146} that finding MIS requires $O(\log n)$ rounds. 

On the other side, to gather global information at all nodes it takes at least $D$ rounds, since the farthest node could be as much as $D$ distance away. Thus, the complexity of algorithms which require global information is $\Omega(D)$. 

Simple problems like finding the count of the number of nodes in the network, constructing a BFS tree, leader election etc are problems which require global information and takes $O(D)$ rounds. Apart from this, there are some problems which require global information and have been proved to take at least $\Omega(D + \sqrt{n})$ rounds. A prominent example is that of finding a Minimum Spanning Tree (MST). It has been shown that to even find an approximate MST we require $\Omega(D + \sqrt{n})$ rounds \citep{DasSarma:2011:DVH:1993636.1993686}. One of the key idea used in most of the algorithms which take $O(D + \sqrt{n})$ is a result from \citep{Kutten:1998:FDC:296903.296906}, which gives a distributed algorithm that can partition nodes of any spanning tree $T$ into $O(\sqrt{n})$ subtrees such that each subtree has $O(\sqrt{n})$ diameter. Basically this approach can be considered as a classical divide and conquer paradigm of distributed algorithms. To solve any problem nodes are divided into $O(\sqrt{n})$ clusters and then the problem is solved in each of the clusters and subsequently, a mechanism is given to combine the result.

\subsection{Overview of past results}
In this section, we will give an overview of the current progress in finding a min-cut. A more detailed technical review of the relevant historical results will be given in next chapter. 

Several attempts at finding min-cuts in the distributed setting (in the \CONGEST model in particular) have been made in past. These include work by \cite{ahuja1989efficient, thurimella1995sub, tsin2006efficient, DBLP:journals/corr/abs-cs-0602013, pritchard2008fast, nanongkai2014almost,ghaffari2016distributed}. A  decade old result by \cite{pritchard2008fast}, currently stands out as the most efficient way to find min-cut of small sizes in particular of size one. They gave an $O(D)$ round algorithm using random circulation technique for finding min-cuts of size $1$. Their result of finding a min-cut of size one has also been extended to give a Las Vegas randomized algorithms to find min-cut of size 2 in $O(D)$ rounds. But a deterministic analogous of the same is not know.  

More recently \cite{nanongkai2014almost} have given a $O((\sqrt{n} \log^* n + D)k^4 \log^2 n)$\footnote{$\log^* n$ (usually read "log star"), is the number of times the logarithm function must be iteratively applied before the result is less than or equal to $1$} rounds algorithm to find min-cut of size $k$. Also, \cite{ghaffari2016distributed} have given a min-cut algorithm for planar graphs which finds a $(1-\epsilon)$ approximate min-cut in $\widetilde{O}(D)$ rounds \footnote{$\widetilde{O}$ hides  logarithmic factors}. In the centralized setting, a linear time algorithms have been proposed for finding min-cut by \cite{kawarabayashi2015deterministic} and improved by \cite{Henzinger:2017:LFP:3039686.3039811}. While a linear time algorithm for finding min-cut exists in the centralized setting, in distributed setting the best know algorithm still takes $O((\sqrt{n} \log^* n + D)k^4 \log^2 n)$ rounds to deterministically find a min-cut of size $k > 1$. Moreover, a $\widetilde{O}(D)$ round algorithm exists to find a min-cut in planar graphs. The following question arises: Is $\Omega(\sqrt{n} + D)$ a lower bound for finding min-cuts or can we save the large factor of $\sqrt{n}$ as known for a planar graph. We answer this question through our thesis. We present new techniques to deterministically find all the min-cuts of size 1,2 and 3. For min-cut of size 1,2 our algorithm takes $O(D)$ rounds and for min-cut of size $3$ our algorithm takes $O(D^2)$ rounds.



==> synopsis_subparts/sketching.tex <==
We introduce a \emph{Sketching} technique for finding min-cuts of size 3. Recall that we have arbitrarily chosen a BFS tree $\tree$. A min-cut of size $3$, if it exists could either 1,2 or 3 respects the tree $\tree$. When a min-cut of size $3$, 1-respects the tree $\tree$, then there exists some node $v$, such that $\eta(v) = 3$. 

To find a min-cut of size 3 which 2 or 3 respects the $\tree$, we will use our characterization lemmas as given in Lemma \ref{lemma:gen_3_cut_2_respect} and  Lemma \ref{lemma:gen_3_cut_3_respect}. Based on these two Lemmas, for any node $u$ if the edge $(\parent u,u)$ is part of min-cut of size $3$, then it requires certain information from other nodes.
For example if $\curly{(\parent u,u),(\parent{v},{v}),(\parent{w},{w})}$ is a min-cut and if node $u$ makes a decision about it, then it needs to know $\eta(u),\eta(v),\eta(w),\gamma(\desc v,\desc u),$ $\gamma(\desc w, \desc u)$ and $\gamma(\desc v,\desc w)$. We give a sketching technique which enables any node $u$ to narrow down on the set of nodes it needs to explore among all possible nodes in the graph. Our Sketching technique deterministically samples certain nodes in the graph based on some combinatorial properties. Here, we will give a brief summary of our sketch definition. Details and proofs will be deferred to the thesis.

For any node $x$, let $\rho_T(x)$ represent the unique path from root $r$ to the node $x$ in the tree $T$. Further, for any vertex set $A \subseteq V$, let $\mathcal P_T(A) \triangleq \curly{\rho_T(x) \mid x \in A}$. We say that a tree path $\rho_T(x)$ is parallel to a tree edge $e = (a,b)$, if $\desc[T]{x} \cap \desc[T]{a} = \emptyset$ and $\desc[T]{x} \cap \desc[T]{b} = \emptyset$. Also for any vertex set $A \subset V$ and a tree $T$ let $\overline{\mathcal N}_T(A) \triangleq \curly{y \mid x \in A, (x,y) \in E, (x,y)\text{ is a non-tree edge}}$. For any two nodes $v_1,v_2$, let $LCA_{T}(v_1,v_2)$ be the lowest common ancestor of node $v_1$ and $v_2$ in tree $T$. Let $firstBranchNode(T')$ of any rooted tree $T'$ is the branch node (a node which has at least two children in a tree $T'$ is called a branch node) closest to root. If the tree $T'$ has no branch node then $firstBranchNode(T')$ is the root itself.
\begin{defn}[Canonical Tree]
\label{defn:sketch_tree}
Canonical tree of a node $v$ is a subtree of some spanning tree $T$ denoted by $R_{T}(v)$ is formed by union (graph-union operation) of tree paths in $\mathcal P_T\paren{\curly{v \cup \overline{\mathcal N}_T\paren{\curly{v}}}}$. Similar to this, the canonical tree of a vertex set $\desc[T]{v}$ is denoted by $R_{T}(\desc[T]{v})$ and formed by union of the paths in $\mathcal P_T\paren{\curly{v \cup \overline{\mathcal N}_T(\desc[T]{v})}}$. Further if node $v$ is some internal node in tree $T$ then for some $c \in \desc[T]{v}$ we define the reduced canonical tree denoted by $R_{T}(\desc[T]{v}\setminus \desc[T]{c})$ is formed by union of the paths in $\mathcal P_T\paren{\curly{v \cup \overline{\mathcal N}_T(\desc[T]{v} \setminus \desc[T]{c})}}$
\end{defn}
We will define sketch as the truncation of the canonical tree and showcase that it can be computed in $O(D^2)$ rounds. In general the canonical tree could be very large in size thus truncation of this is required. The truncation is designed in such a way that if a node $v$ is not present in the truncated canonical tree of some node $u$, then the edge $(\parent v,v)$ may not take part in the min-cut containing the edge $(\parent{ u},{u})$. To characterize this kind of truncation we will use branching number as defined in Definition \ref{defn:branching_number}. We will defer the details to the thesis. 

\begin{defn}[Branching Number]
\label{defn:branching_number}
For any tree $T'$, the branching number of a node $b$ in tree $T'$ is denoted by $\bnum[T']{b}$ and is defined as
$$\bnum[T']{b} \triangleq  \begin{cases}
1& \level[T']{b} \leq  \level[T']{x}\\
deg_{_{T'}}(\parent[T]{b}) + \bnum[T']{\parent[T']{b}} - 2& \level[T']{b} > \level[T']{x}\\
\end{cases}
$$
where $x = firstBranchNode(T')$
\end{defn}

We make the following simple observation about branching number and give a characterizing lemma regarding the size of the canonical tree. Their proofs are deferred to the thesis.
\begin{obs}
\label{obs:branchin_number_increases}
Let $v$ be a node and $c \in \child_T(v)$. Let $b \in R_T(\desc[T]{c})$, then $\xi_{R_T(\desc[T]{c})}(b) \leq \xi_{R_T(\desc[T]{v})}(b)$.
\end{obs}
\begin{lemma}
For any tree $T'$, the number of nodes in the tree that has branching number less than $k$ is $O(2^k Depth(T'))$
\label{obs:nodes_R_t_v}
\end{lemma}
Our graph sketch of a node is defined based on the canonical tree and comes with a parameter $k$ on which the truncation is based. Our graph sketch will be called as $k$-Sketch. A meta information about each node is also added in $k$-Sketch. Before defining $k$-sketch we define the trimming of tree.

\begin{defn}[trunc]
For some tree $T'$ and a number $k$, $trunc(T',k)$ is an sub-tree of $T'$ induced by vertices with branching number less than or equal to $k$.
\end{defn}
\begin{defn}[$k$-Sketch]
\label{defn:k_sketch}
For any node $v$ and a spanning tree $T$, let $R' =  trunc(R_T(\desc[T]{v}),k)$. The $k$-Sketch of a node $v$ w.r.t. the spanning tree $T$ is denoted as $\Sketch[T]{k}{v}$ and it is defined as $\Sketch[T]{k}{v} \triangleq \curly{R' \cup \curly{\angularbracs{u:\eta_{T}(u),\parent[T]{u},\gamma\paren{\desc[T]{v},\desc[T]{u}}}\ \forall u \in R'}}$
\end{defn}
Basically $k$-Sketch is a truncated canonical tree packaged along with the meta information $\angularbracs{u:\eta_{T}(u),\parent[T]{u},\gamma\paren{\desc[T]{v},\desc[T]{u}}}$ for each node $u$ in the truncated tree. This is designed is such a way that all the information required as per Lemma \ref{lemma:gen_3_cut_2_respect} and Lemma \ref{lemma:gen_3_cut_3_respect} are present. We now give the following Lemma about the size of the $k$-Sketch.
\begin{lemma}
For some spanning tree $T$ and a fixed $k$, the $k$-Sketch of a node $v$, $\Sketch[T]{k}{v}$ w.r.t. $T$ is of size $O(Depth(T) \log n)$ bits.
	\label{lemma:size_sketch}
\end{lemma}
We will compute the $k$-Sketch w.r.t the fixed BFS tree $\tree$ and omit $\tree$ from the subscript of the sketch notation.
\begin{lemma}
For all $v \in V$ and a fixed $k$, $\Sketch{k}{v}$ can be computed in $O(D^2)$ rounds.
\label{lemma:k-sketch_algorithm}
\end{lemma}
We will compute the sketch for $k=2,3$. We also define \emph{reduced sketch} which is a variant of the above defined sketch and \emph{layered algorithm} in the thesis. These techniques put together will enable us to find all the min-cuts of size 3.

\begin{thm}
 There exists a $O(D^2)$ round distributed algorithm which deterministically finds all min-cuts of size 3.
\end{thm}

==> synopsis_subparts/techBackground.tex <==
In this section, we will review some past results for finding min-cuts, in particular, the ideas employed in two recent works \citep{nanongkai2014almost,pritchard2008fast}. While \cite{nanongkai2014almost} relied on greedy tree packing introduced by \cite{thorup2001fully}; \cite{pritchard2008fast} gave a novel technique of random circulations.
\paragraph{Greedy Tree Packing based technique:}
First, we will define the concept of greedy tree packing. A \emph{tree packing} $\mathbb{T}$ is a multiset of spanning trees. Let the load of any edge $e$ w.r.t a tree packing $\mathbb{T}$ denoted 
by $\mathcal L^{\mathbb{T}}(e)$, be defined as the number of trees in $\mathbb{T}$ containing $e$. A tree packing $\mathbb{T} =\curly{T_1,\ldots, T_j}$ is greedy if each $T_i$
is a minimum spanning tree (MST) with respect to the loads induced by $\curly{T_1,\ldots, T_{i-1}}$. \cite{thorup2001fully} has given the following results related to tree packing:

\begin{thm}[\cite{thorup2001fully}]
Let $G = (V,E)$ be an unweighted graph. Let $m$ be the number of edges in $G$ and $k$ be the size of min-cut. Then a greedy tree-packing with $\omega(k^7 \log ^3 m)$ contains a tree crossing some min-cut exactly once.
\label{thorup-tree-packing}
\end{thm}
Based on the above theorem, \cite{nanongkai2014almost} construct a greedy tree packing of $\omega(k^7 \log ^3 m)$ trees. There is a well-known algorithm to find MST in $O(D + \sqrt{n})$ rounds. Further, in each tree, the authors find the size of the smallest edge cut which shares only one edge with the tree. They give an algorithm to do the same in $O(D + \sqrt{n})$ rounds for each tree. Note that they cannot find all the min-cuts because of the limitations of Theorem \ref{thorup-tree-packing}.


\paragraph{Random Circulation based technique:}
The random circulation technique has its foundation based on a well known fact that cut spaces and cycle spaces are orthogonal to each other \citep{bondy1976graph}. Based on this technique \cite{pritchard2008fast} is able to give the following result
\begin{thm}[\cite{pritchard2008fast}]
There is a Las Vegas distributed algorithm to compute all the min-cuts of size 1 and 2 (cut edges, cut pairs respectively) in $O(D)$ time.
\end{thm}



==> synopsis_subparts/trsf.tex <==

\label{subsec:intro_trs}
In this section we define \textit{tree restricted semigroup function} and demonstrate a simple and natural application of it in finding induced-cuts of size 1. A more advanced application to find induced cuts of size $2$ will be given in the thesis. A tree restricted semigroup function is defined with respect to a tree $T$ and based on a commutative semigroup.  Recall that a commutative semigroup is a set $\mathcal X$ together with a commutative and associative binary operation $\boxplus$ which is a function $\boxplus: \mathcal{X} \times \mathcal{X} \rightarrow \mathcal{X}$. {Tree restricted semigroup function} is inspired by semigroup function defined by Peleg in \cite[Def. 3.4.3]{peleg2000distributed}.

Let $\mathcal X$ be a commutative semigroup with operator $\boxplus$. Let $T$ be any spanning tree. We will define $f : V \rightarrow \mathcal X$ to be a tree restricted semigroup function with respect to the tree $T$ in Defn \ref{defn:restricted_semigroup_function}. Let $a \in V$ be any node. For each $v \in \ancestor[T]{a}$, node $a$ computes the value $X_{a}^{v}$ through a distributed algorithm (mainly as a pre-processing step), which is the contribution by node $a$ for calculating tree restricted semigroup function $f(v)$. 
\begin{defn}[Tree Restricted Semigroup function]
\label{defn:restricted_semigroup_function}
Let $\mathcal X$ be a commutative semigroup with the operator $\boxplus$. Then, the function $f : V \rightarrow \mathcal X$ is a tree restricted semigroup function if $f(v) = \bigboxplus\limits_{a \in \desc[T]{v}} X_{a}^{v}$.
\end{defn}
In the above definition, $X_{a}^{v} \in \mathcal X$ for some node $a$ and all $v \in \ancestor[T]{v}$ is an atomic value computed by node $a$ based on the properties of $f(\cdot)$.
Further, for any $a \in V$ and $v \in \ancestor[T]{a}$, define $X_{\desc[T]{a}}^{v} = \bigboxplus\limits_{a' \in \desc[T]{a}} X_{a'}^{v}$. Note that $X_{\desc[T]{a}}^{v} \in \mathcal X$. We will say that $X_{\desc[T]{a}}^{v}$ is the contribution of nodes in the set $\desc[T]{a}$ for computing $f(v)$.
\begin{obs}
\label{obs:info_required_to_aggregate}
 Let $a$ be an internal node in the tree $T$ and $v \in \ancestor[T]{a}$ then $$X_{\desc[T]{a}}^{v} = X_{a}^{v} \boxplus \paren{\bigboxplus\limits_{c \in \child(a)} X_{\desc[T]{c}}^{v}}$$ \end{obs} 
\begin{obs} 
\label{obs:info_required_to_compute_trsf}
For any internal node $v$
$$f(v) = X_{v}^{v} \boxplus \paren{\bigboxplus\limits_{c \in \child(v)} X_{c^\downarrow}^{v}}$$ 
\end{obs}

\begin{defn}
A tree restricted semigroup function $f(\cdot)$ w.r.t to a tree $T$ is efficiently computable if for all $v$, $f(v)$ can be computed in $O(Depth(T))$ time in the \CONGEST model.
\end{defn}
In Lemma \ref{lemma:tree_restricted_semigroup_function},  we will give sufficient conditions for a tree restricted semigroup function to be efficiently computable. An algorithmic proof of which is given in the thesis. 
\begin{lemma}
\label{lemma:tree_restricted_semigroup_function}
For all $a \in V$ and $v \in \ancestor[T]{a}$ if $X_a^v, X_{\desc[T]{a}}^v, f(v)$ are all of size $O(\log n)$ bits and if the atomic value $X_a^v$ can be computed in $O(Depth(T))$ time by node $a$ then the tree restricted semigroup function $f$ is efficiently computable.
\end{lemma}

We will now demonstrate a small application of tree restricted semigroup function. For any node $v$ we define tree cuts as the cut induced by the vertex $\desc[T]{v}$. The size of tree cut is a function $\eta_T: V \rightarrow [m]$ where $\eta_T(v) = |\delta(\desc[T]{v})|$. We will work with an arbitrary fixed BFS tree $\tree$. For any node $a$ and $v \in \ancestor{a}$ we will use $H_{a}^{v}$ equal to the number of  vertices adjacent to $a$ which are not in vertex set $\desc{v}$. The commutative semigroup associated here is the set of all positive integers $\mathbb Z^+$ with the operator "+". We give the pre-processing steps in Algorithm \ref{algo:preprocessing-cut-1-respects-tree} which calculates $H_{a}^{v}$ for all $v \in \ancestor{a}$. 

\begin{algorithm}[h]
\DontPrintSemicolon
\SetKwFor{Forp}{for}{parallely}{endfor}
\lForp{$b$ adjacent to $a$}{send the ancestor set $\ancestor{a}$ to $b$} 
\lForp{$b$ adjacent to $a$}{receive the ancestor set $\ancestor{b}$} \label{line:pre-processing-eta-v-communication} 
\For{$v \in \ancestor{a}$}{
	$H_{a}^{v} \gets |\curly{b\mid (a,b)\in E,\ v\notin \ancestor{b}}|$\;
	\tcc{node $a$ can execute the above step locally because it knows $\ancestor{b}$, $\forall\ (a,b) \in E$}
}
\caption{Pre-Processing for computing the function $\eta$ (run at all node $a$ for finding $H^{v}_{a}\ \forall\ v \in \ancestor[T]{a}$)}
\label{algo:preprocessing-cut-1-respects-tree}
\end{algorithm}
\begin{obs}
\label{prepo:pre-processing-size-tree-cuts}
Pre processing as given in Algorithm \ref{algo:preprocessing-cut-1-respects-tree} takes $O(D)$ time.
\end{obs}
\begin{proof}
Any node $a$ has at most $D$ ancestors in $\tree$. So for every node $b$ adjacent to $a$, it takes $O(D)$ time to communicate the set $\ancestor{a}$ to it similarly it takes $O(D)$ time to receive the set $\ancestor{b}$ from node $b$. Now $H_{a}^{v}$ for any $v \in \ancestor{a}$ will just be an internal computation at node $a$. 
\end{proof}

\begin{lemma}
For any node $v\in V$ and $a \in \desc{v}$, $\eta(v)$ and $H_{\desc{a}}^{v}$ can be computed in $O(D)$ time 
\end{lemma}
\begin{proof}
In Lemma \ref{lemma:eta_v_is_restricted_semigroup_function}, we show that $\eta$ is an efficiently computable {tree restricted semigroup function}. We work with BFS tree $\tree$ such that $Depth(\tree)$ is  $O(D)$. Thus $\eta$ can be computed in $O(D)$ time for all $v \in V$ also during the process of computation of each node $a \in \desc{v}$ computes $H_{\desc{a}}^{v}$.
\end{proof}
\begin{lemma}
\label{lemma:eta_v_is_restricted_semigroup_function}
$\eta(\cdot)$ is an efficiently computable {tree restricted semigroup function}.
\end{lemma} 
\begin{thm}
\label{theorem:1-cuts}
There exists a $O(D)$ round distributed algorithm which deterministically finds all edge-cuts.
\end{thm}
\begin{proof}
To find if there exists a min-cut of size $1$ each node $v$ checks if $\eta(v) = 1$. This is sufficient because if there exists an edge $e$ such that removal of it disconnects the graph and partitions the vertex into two, then it will be part of all trees. For some node $v$, let $e = (\parent{v},v)$ be such an edge. Removal of $e$ partitions the vertex set into $\desc{v}$ and $V\setminus \desc{v}$. Thus there is no edge apart from $(\parent{v},v)$ which goes out of the vertex set $\desc{v}$ and hence $\eta(v) = 1$. 
\end{proof}

The above demonstrated application of TRSF is very simple. A more appreciable application of TRSF is its power to find min-cuts of size $2$. Through TRSF, we just need to define atomic values and prove that those can be computed through a distributed algorithm in a fast and efficient manner. We then have to give guarantees about the possible bit-sizes of such atomic values. Then using Lemma \ref{lemma:tree_restricted_semigroup_function}, we can guarantee that the underlying tree restricted semigroup function is efficiently computable.

Similar to $\eta(\cdot)$, for finding min-cuts of size $2$ we will define another tree restricted semigroup function $\zeta : V \rightarrow \mathcal Z$ where $\mathcal Z$ is a specially designed semigroup where each element is a four tuple and a special operator $\odot$. Similar to $H_{a}^{v}$, we show that the underlying atomic values $Z_{a}^{v}$, for any node $a$ and $v \in \ancestor{a}$, can be found in $O(D)$ rounds via a preprocessing algorithm. Details about the definitions of $\zeta(\cdot)$ and the atomic value $Z_{a}^{v}$ are given in the thesis. The function $\eta(\cdot),\zeta(\cdot)$ and $H_{\desc a}^{v}$ and $Z_{\desc a}^{v}$ helps us find all the required quantities as per Lemma \ref{lemma:2-respect-2-cut} for any possible min-cut of size 2. Using this we can prove the following theorem. 
 \begin{thm}
 \label{theorem:2-cuts}
 There exists a $O(D)$ round distributed algorithm which deterministically finds all min-cuts of size 2.
 \end{thm}
